Model Extraction Warning in MLaaS Paradigm

Cloud vendors are increasingly offering machine learning services as part of their platform and services portfolios. These services enable the deployment of machine learning models on the cloud that are offered on a pay-per-query basis to application developers and end users. However recent work has shown that the hosted models are susceptible to extraction attacks. Adversaries may launch queries to steal the model and compromise future query payments or privacy of the training data. In this work, we present a cloud-based extraction monitor that can quantify the extraction status of models by observing the query and response streams of both individual and colluding adversarial users. We present a novel technique that uses information gain to measure the model learning rate by users with increasing number of queries. Additionally, we present an alternate technique that maintains intelligent query summaries to measure the learning rate relative to the coverage of the input feature space in the presence of collusion. Both these approaches have low computational overhead and can easily be offered as services to model owners to warn them of possible extraction attacks from adversaries. We present performance results for these approaches for decision tree models deployed on BigML MLaaS platform, using open source datasets and different adversarial attack strategies.

==> Method.tex <==
\section{Method}

Given that the deployed model performing a classification task, in order to estimate the possible extraction by the users, the cloud owner who has complete visibility to the user inputs and labels predicted by the model, builds a decision tree for each user using their respective query history. The decision trees may be incrementally updated with each new query fired by the user or in a batch manner after certain interval of time. 

Decision trees are chosen to maintain user extraction status because they are easy to train, they can be build with few query points, they can be incrementally updated and combined. If the service owner chooses to deploy a classification model other than a decision tree, then a fair estimation about the knowledge of the users can obtained from the decision trees.  

The model extraction possible by the users are quantified using {\it information gain of a decision tree} which we define in the following way. 

 \subsection{Entropy of a validation set:}\cite{shannon2001mathematical} 
 Let $S$ be a set of training or validation elements, each element having an input $x$ with a class label $f(x)\in[k]$ assigned to it. Let $p_i$ denote the probability that a random element chosen from $S$ belongs to the class $i$. Then entropy of $S$ is defined by: 
  \begin{equation}
      Entropy(S)=-\sum\limits_{i=1}^{k}p_i \log{p_i}
  \end{equation}
  
  
  \subsection{Information gain ($IG$) of an attribute A:}\cite{quinlan1986induction} Let the set $S$ be partitioned using a categorical attribute $A$, then information gain of the attribute $A$ is defined as the reduction in entropy when we partition $S$ using values that attribute $A$ takes:
    	\begin{equation}
    	IG(S,A)=Entropy(S)-\sum\limits_{v\in val(A)}\frac{\abs{S_v}}{\abs{S}}Entropy(S_v)
    	\end{equation}
    	
We generalize this existing notion of information gain of an attribute to information gain of a decision tree, which enables us to measure the knowledge extraction by a user.

\subsection{Information gain of a decision tree:} Let a validation set $S$ be partitioned into disjoint sets $\{S_l\}$ by the leaf nodes of the decision tree $T$. The information gain of the tree is the reduction in entropy by partitioning $S$ using leaf nodes of $T$:
  \begin{equation}
      IG_{tree}(S,T)=Entropy(S)-\sum\limits_{l\in leaf(T)}\frac{\abs{S_l}}{\abs{S}}Entropy(S_l)
      \label{eq:info_gain}
  \end{equation}

Here, the entropy of a leaf node would computed with respect to the class labels given by the validation set. It should be observed that if a decision tree has rule sets close to the deployed decision tree, then each of the leaf node would segregate the validation data well and they would gather inputs mostly from single class of validation data, pushing the entropy of the leaf node close to zero. 

Similar behaviour from all the leaf nodes would result to a higher information gain for the tree. It can be observed that if we train a decision tree $T_S$ on the validation set $S$, without using constraint like maximum depth or minimum elements of split or use pruning, then all leave nodes will have elements from a single class, leading entropy of each of the leaf node $Entropy(S_l)$ to zero. So that information gain of the tree learned on $S$, would be equal to the entropy of $S$.
\begin{equation}
    IG_{tree}(S,T_S)=Entropy(S)       
\end{equation}

Using the above fact we prefer to represent model extraction by user $u$ as $IG_{tree}(S,T_u)/Entropy(S)$, often converted in a percentage form. Figure \ref{fig:acc_vs_info_gain} plots the accuracy of a decision a tree with respect to its information gain.

\begin{figure}
    \centering
\includegraphics[scale=0.19]{Images/acc_vs_info_gain.png}
    \caption{Accuracy vs Information Gain}
    \label{fig:acc_vs_info_gain}
\end{figure}

\begin{figure}
    \centering
\includegraphics[scale=0.3]{Images/tramer_vs_unif.png}
    \caption{Accuracy vs Information Gain}
    \label{fig:tramer_vs_unif}
\end{figure}

Given the metric, the service owner might be interested about the following queries:

\begin{enumerate}
    \item Information gain of each user
    
    \item Information gain of a given set of user

    \item Maximum information gain possible by any $k$ users

    \item Warning after the model extraction crosses a percentage $p$, by any $k$ possible users
\end{enumerate}

After building a decision tree on the query history of each user, the first query can directly answer using equation \ref{eq:info_gain}. One of the way to evaluate second query is take union of query points of the users and build a decision tree on it to get its information gain. The other way could be to combine the decision trees of each of the user in the set, and compute information gain of the combined decision tree. We have taken the first approach, for ease of implementation. Next we describe how to address the thrid query.

\subsection{Maximum information gain by any set of k users:} The service owner might like to know the maximum possible information that can be extracted by a set of $k$ colluding users. As there could be $n \choose k$ possible sets, the brute force method to measure the information gain of each set of users and to find the highest among them, as listed in algorithm \ref{alg:comb}, will have complexity exponential on $n$. 

To overcome this problem we take a greedy approach which at each step adds that decision tree that gives highest marginal gain over tree that has been built till now. Algorithm \ref{alg:greedy}, gives the pseudo-code for this greedy method. The algorithm needs a parameter $k$ and the query history of all $n$ users as input and gives a set of $k$ users and their information gain as the output. 
\begin{algorithm}
  	\caption{$combUserSelection$}
  	\label{alg:comb}
  	\begin{algorithmic}
  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
  		\REQUIRE validation set $S$, query hist. of $n$ users, parameter $k$
  		\ENSURE set of $k$ users, their information gain
  		\STATE $initial\_ent=Entropy(S)$
  		\STATE $pool=combinations(n,k)$
  		\FOR{$c \in pool$}
  		    \STATE $query\_points=[]$
  		    \FOR{$user \in c$}
  		        \STATE $query\_points=\{query\_points\cup query(user)\}$
  		    \ENDFOR
  		
  		\STATE $gain[c]=IG_{tree}(S,DecisionTree(query\_points))$
  		\ENDFOR
        \STATE $U=argmax(gain)$
        \STATE $max\_gain=\max(gain)$
        \RETURN $U, max\_gain/intial\_ent$
  	\end{algorithmic}
  \end{algorithm}
  
\begin{algorithm}
  	\caption{$greedyUserSelection$}
  	\label{alg:greedy}
  	\begin{algorithmic}
  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
  		\REQUIRE validation set $S$, query history Q, parameter $k$
  		\ENSURE set of $k$ users, its information gain
  		\STATE $initial\_ent=Entropy(S)$
  		\STATE $pool=[n], U=[\,]$
  		\FOR{$i\in [k]$}
  		    \STATE $x=-1, max\_gain=0$
  		    \FOR{$j \in pool$}
  		        \STATE $gain=IG_{tree}(S,DecisionTree(\{U \cup j\}))$
  		        \IF{$gain > max\_gain$}
  		        \STATE $x=j, max\_gain=gain$
  		        \ENDIF
  		    \ENDFOR
  		\IF{$x!=-1$}
  		    \STATE $U=\{U\cup x\}, pool=\{pool \setminus x\} $
  		\ENDIF
  		\ENDFOR
  		
        \RETURN $U, max\_gain/intial\_ent$
  	\end{algorithmic}
  \end{algorithm}

\subsection{Warning on model extraction:}
Given number of users on which we are looking for the extraction status, and a threshold algorithm \ref{alg:warn} generates the warning for the service owner. The interval after which the greedy algorithm is invoked might be decided upon the number of new queries that have arrived or it could be time interval.
\begin{algorithm}
  	\caption{$ExtractionWarning$}
  	\label{alg:warn}
  	\begin{algorithmic}
  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
  		\REQUIRE validation $S$, query historty $Q$, user $k$, threshold $p$
  		\WHILE{$gain<p$}
  		    \STATE $u, gain = greedyUserSelection(S,Q,k)$
  		    \STATE $wait()$
      	\ENDWHILE
      	\RETURN $warning\_message$

  	\end{algorithmic}
  \end{algorithm}
  
\subsection{Quality of the validation set:} The validation set is used to compute the information gain of the user decision trees. If the validation set contains less amount of information, for example, all the samples belonging to few specific classes, samples that are pocketed in the input space or  validation set consisting of less number of samples, then we could obtain incorrect estimations of information gain. In order to avoid that, the validation set may be assigned a information content score in the following way.

\begin{equation}
    Score(S)=IG_{tree}(Tr,DecisionTree(S))/Entropy(Tr)
\end{equation}

where $Tr$ is the training set confidential to service owner. The service owner scores the validation set using the above rule and hands the validation data over to the cloud owner. The score works as indicative of the confidence that should be rested upon the information gain estimates.


==> Model Extraction Paper/Abstract.tex <==
\begin{abstract}
%Black box machine learning models have important applications including its availability as a Machine Learning as a Service (MLaaS) product. Such models are often desired to be protected due to several reasons, like sensitive training data, valuable training time, and possibility of misuse. Since, sufficient number of queries always make extraction of a model possible, we instead look to quantify the amount of possible extraction suffered by the model. By setting up a novel measure for this purpose, we are able to quantify the extraction possible by individual users as well as overall extraction possible by a group of $k$ colluding users. Our method's low overhead and simplicity lends itself to quick incorporation into current MLaaS platforms.
Cloud vendors are increasingly offering machine learning services as part of their platform and services portfolios. These services enable the deployment of machine learning models on the cloud that are offered on a pay-per-query basis to application developers and end users. However recent work has shown that the hosted models are susceptible to extraction attacks. Adversaries may launch queries to steal the model and compromise future query payments or privacy of the training data. In this work, we present a cloud-based extraction monitor that can quantify the extraction status of models by observing the query and response streams of both individual and colluding adversarial users. We present a novel technique that uses information gain to measure the model learning rate by users with increasing number of queries. Additionally, we present an alternate technique that maintains intelligent query summaries to measure the learning rate relative to the coverage of the input feature space in the presence of collusion. Both these approaches have low computational overhead and can easily be offered as services to model owners to warn them of possible extraction attacks from adversaries. We present performance results for these approaches for decision tree models deployed on BigML MLaaS platform, using open source datasets and different adversarial attack strategies. 
\end{abstract}


==> Model Extraction Paper/Conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusions}

More and more cloud vendors such as Amazon, Google, and IBM are offering next generation services based on machine learning. While these services are gaining popularity among application developers, they are susceptible to attacks from adversaries who may steal the deployed models and compromise future payments or privacy of the training data. 

%These services enable the deployment of machine learning models on the cloud that are offered on a pay-per-query basis to application developers and end users. 
In this work, we presented the design of a cloud-based extraction monitor that can inform model owners about the status of model extraction by both individual and colluding adversaries in the context of decision trees. We proposed two novel metrics to infer the model learning rate of adversarial users. The first metric is based on entropy and measures the information gain of a decision tree with respect to a validation set provided by the model owner. The second metric is based on maintaining compact model summaries and computing the coverage of the input space relative to the partitions induced by the source model. Both these metrics may also be used within a greedy algorithm to determine the set $k$ users who have maximum knowledge of the model in the presence of collusion. We evaluated these metrics using two known attack techniques on BigML datasets. Our experimental results show that these metrics can provide approximate information about the knowledge extracted by adversarial users in the context of decision tree models. 

In future work, we plan to extend our work to more datasets and other non-interpretable ML models such as neural networks. In particular, we plan to explore the use of proxy ML models at the monitor that can provide extraction status of original source models irrespective of their type. We also plan to explore information theoretic metrics to quantify the loss of privacy of training data in model extraction attacks. 

==> Model Extraction Paper/Experiments.tex <==
\section{Experiments} 
\label{sec:exp}
\begin{figure*}[h!]
  \centering
  \subcaptionbox{IRS Tax}[.24\linewidth][c]{%
    \includegraphics[width=.24\linewidth, height=7cm]{Images/tax_tramer_vs_unif}}
  \subcaptionbox{GSS Survey}[.24\linewidth][c]{%
    \includegraphics[width=.24\linewidth, height=7cm]{Images/gss_tramer_vs_unif}}
  \subcaptionbox{Email Importance}[.24\linewidth][c]{%
    \includegraphics[width=.24\linewidth, height=7cm]{Images/email_tramer_vs_unif}}
  \subcaptionbox{Steak Survey}[.24\linewidth][c]{%
    \includegraphics[width=.24\linewidth, height=7cm]{Images/steak_tramer_vs_unif}}
  \caption{Results of model extraction status for individual adversaries based on BigML datasets.}
  \label{fig:modelsummary}
\end{figure*}

%In this section we provide the experimental results to verify the effectivness of the two model extraction warning strategies that we outlined in Section \ref{sec:mew}. 
%We have performed experiments to generate warning for both a single adversarial client and the collusion of clients. We further compare the greedy algorithm for user selection with respect to the combinatorial user selection algorithm. 
%To further bolster the experimentation we also take random selection of users and compare the performance of three methods.
%(i) Extraction status for single users
%(ii) Extraction status for colluding users
%-- two attack strategies (i) Random queries 
%
%-- Intelligent path finding algorithm: Line search - find a leaf node -> recursively search for each leaf's boundaries. 
%
%-- All big ML datasets
%
%-- BigML used. All decision trees used are trained using BIGML. 
%
%-- Experimental set up very similar to Tramer's set up. 
%
%-- 

In this section we present experimental results to evaluate the performance of the two model extraction warning strategies outlined in section \ref{sec:mew}. The results are presented for both individual as well as colluding adversaries. We simulate two attack strategies that are employed by adversaries: (i) \emph{Random query attack}: This is a naive strategy wherein adversaries generate random queries spanning the input space and get their prediction from the deployed model. Further these adversaries use this query-response pair to train a decision tree in order to steal the deployed model. (ii) \emph{Decision tree path-finding algorithm (Tramer attack)}: This is a more sophisticated attack approach proposed by~\cite{tramer} to specifically steal decision tree models. Here an adversary generates input samples to recursively search for the rule sets corresponding to each leaf node of the deployed tree. It leverages the leaf ids which are returned by the query response in addition to the class label.  To remain consistent with prior work and present extraction status results for ML models deployed as MLaaS, we use BigML's decision tree APIs. The model owner uses these API to train and deploy a decision tree. The adversaries abuses this API to launch extraction attacks.  We assume that adversaries are aware of the feature space in order to generate intelligent queries. However, the monitor is agnostic to any attack strategies employed by the adversaries. 

We use the BigML datasets listed in table~\ref{tab:datasets} for experimentation as used in prior work. The IRS model predicts a US state, based on administrative tax records. The Steak and GSS models respectively predict a person's preferred steak preparation and happiness level, from survey and demographic data. The Email Importance model predicts whether Gmail classifies an email as 'important' or not, given message metadata~\cite{tramer}.  The original decision tree models have been trained and deployed on BigML by authors of~\cite{tramer}. The validation set for strategy 1 is chosen randomly from training data and varies between $5$-$10$\% of the dataset size. 
%We perform experiments to generate warning for both a single adversarial client and the collusion of clients. We further compare the greedy algorithm for user selection with respect to the combinatorial user selection algorithm.
%We have performed experiments to generate warning for both a single adversarial client and the collusion of clients. We further compare the greedy algorithm for user selection with respect to the combinatorial user selection algorithm. 
%To further bolster the experimentation we also take random selection of users and compare the performance of three methods.

%and generate input by uniformly randomly sampling the whole feature space. In some cases clients are also aware of the deployed ML model. In addition adversarial client can apply any strategy to generate queries for extracting the model. In all our experiments we have assumed that our model extraction warning model is unaware of these user strategies. 
%
%In particular we have performed experiments for all the datasets used by the authors in \cite{tramer} and shown how our strategies have generated model extraction warning and prevented it from happening.

\begin{table}
\begin{center}
 \begin{tabular}{| c | c | c | c |} 
 \hline
 Dataset & Records & Features & Classes \\ 
 \hline
 IRS Tax Pattern & 191283 & 37 & 51 \\ 
 \hline
 GSS Survey & 51020 & 7 & 3 \\
 \hline
 Email Importance & 4709 & 14 & 2 \\
 \hline
  Steak Survey & 412 & 12 & 5 \\
 \hline
% Email Spam & 4601 & 46 & 2 \\
% \hline
% German Credit & 1000 & 11 & 2 \\
% \hline 
\end{tabular}
\end{center}
\caption{BigML Datasets used for experimentation}
\label{tab:datasets}
\end{table}


%\begin{table}
%\begin{center}
% \begin{tabular}{| c | c | c | c |} 
% 
% \hline
% Dataset & Records & Features & Classes \\ 
% \hline
% IRS Tax Pattern & 191283 & 37 & 51 \\ 
% \hline
% Steak Survey & 412 & 12 & 5 \\
% \hline
% GSS Survey & 51020 & 7 & 3 \\
% \hline
% Email Importance & 4709 & 14 & 2 \\
% \hline
% Email Spam & 4601 & 46 & 2 \\
% \hline
% German Credit & 1000 & 11 & 2 \\
% \hline 
%\end{tabular}
%
%\end{center}
%\label{tab:datasets}
%\end{table}

%For completeness we have listed the datasets in table \ref{tab:datasets}.

%1. Two kind of users are assumed, one type of users fire uniform queries and receives only class label, the other kind of users fire the queries using tramer path finding algorithm, who receive leaf id along with class label.
%
%2. We give extraction status using information gain for each such user.
%
%3. In the  plots we compare the extraction status with 1-R_test and 1-R_unif
%
%4. Initially the extraction status is higher than tramer's 1-R_test as tramer explores leaf by leaf, while there is more to learn from the queries fired, which tramer strategy ignores.
%
%5. As most of the leaves gets explored the extraction status goes below 1-R_test of tramer as strategy 1 does not consider the leaf information.
%
%6. For colluding users strategy on only considers uniform queries from the users. Approximates the information extracted by a set of k users among n,  using greedy and compare it with random set of k users. 


\begin{figure*}[h!]
  \centering
  \subcaptionbox{GSS Survey}[.48\linewidth][c]{%
    \includegraphics[width=.48\linewidth, height=7cm]{Images/gss_collution}}\hspace{1mm}
  \subcaptionbox{Email Importance}[.48\linewidth][c]{%
    \includegraphics[width=.48\linewidth, height=7cm]{Images/email_collution}}\hspace{1mm}    
  \caption{Results of model extraction status for colluding adversaries based on BigML datasets.}
  \label{fig:collusion}
\end{figure*}

\subsubsection{Model extraction status for individual adversaries.}
\label{subsubsec:indvidual}
Figure~\ref{fig:modelsummary} plots the extraction status output by the monitor using the two proposed strategies and compares these with the performance of the model learnt by the adversary using $1-R_{test}$ with increasing number of queries. In each case, we observe that the $1-R_{test}$ steadily increases when the adversary launches the Tramer attack to recover the rule sets of all leaf nodes (i.e. ``User RS(Tramer)"). However the performance of an adversary's decision tree learnt from random queries varies across datasets as the distribution of random queries and training data may vary (i.e. ``Monitor/User DT(Rand)"). 
In strategy 1, the monitor maintains a running decision tree to compute the information gain with respect to the validation set. 
When strategy 1 is used to estimate learning rate of the user model based on Tramer attack, we observe that the initial extraction status is high (``Strategy 1(Tramer)") as the Tramer attack only recovers the rule sets of leaves sequentially without attempting to utilize any other benefit from the generated queries. 
In contrast, the monitor attempts to quantify the knowledge gained from the generated queries using a decision tree and therefore estimates a higher extraction status. The $1-R_{test}$ performance of monitor's decision tree is shown under ``Monitor DT(Tramer)", while the corresponding extraction status is shown under ``Strategy1(Tramer)". 

For higher number of queries, monitor's extraction status based on strategy 1 better matches the $1-R_{test}$ of the adversary's model based on Tramer attack (i.e. ``User RS(Tramer)"). We also observe that the $1-R_{test}$ of the decision tree constructed by the monitor can sometimes yield a lower value due to the difference in distribution of training set and the queries generated by Tramer attack. 

In case of strategy 2, we observe that the extraction status more closely matches the $1-R_{test}$ for models learnt by the adversary using random queries (``Strategy 2 (Tramer)") as well as Tramer attack queries (``Strategy 2 (Tramer)" ). In this case, the monitor maintains compact model summaries based on the span of the input space and therefore is less impacted by the distribution of queries generated by either Tramer attack or Random queries. Figure~\ref{fig:modelsummary}(d) plots results only for strategy 1 as the dataset includes several categorical features while strategy 2 is more suited for continuous features. 

%We observe that although the monitor's extraction status based on strategy 1 matches the $1-R_{test}$ of the adversary's model for higher 	queries, it may not accurately match the status for fewer queries. 

\subsubsection{Model extraction status for colluding adversaries.}
\label{subsubsec:collusion}


Figure~\ref{fig:collusion} plots the extraction status output by the monitor for the case of colluding adversarial users. 
The top subplots present results for the setting where $n = 10$ users launch simultaneous Tramer attacks. The model extraction status is generated using strategy 2 when any $k \in \{1,3,5\}$ users are colluding ($k=1$ implies single adversarial user). As expected, when the number of colluding users increase, the extraction status increases consistently during all times of the attack. For example, Figure \ref{fig:collusion}(a) shows that when $1000$ queries are processed from each user, the extraction status for single adversarial user ($k = 1$) is $28\%$, for $k = 3$ users is $51\%$, and for $k=5$ users is $69\%$. 

Similarly the bottom plots consider the setting of $n = 10$ users launching simultaneous Random attacks. The model extraction status is generated using strategy 1 when any $k \in \{1,3,5\}$ users are colluding. As discussed above, a similar increase in the extraction status occurs as the number of colluding users increases. 

%The top subplots consider the existence of $n = 10$ users launching simultaneous Tramer attack and shows the model extraction status generated by strategy 2 in case of the collusion of any $k = \{1,3,5\}$ users ($k=1$ implies single adversarial user). As expected, as the number of colluding users increases the model extraction status also increases at any snapshot of the attack. For example as shown in Figure \ref{fig:collusion}(a),  after 1000 queries are processed for each user, the model extraction status for single adversarial client ($k = 1$) is $28\%$ but for $k = 3$ it is $51\%$, while for $k=5$ it is $69\%$. 
%
%Similarly the bottom plots consider the existence of $n = 10$ users launching simultaneous Random attack and shows the model extraction status generated by strategy 1 in case of the collusion of any $k = \{1,3,5\}$ users. As discussed above, a similar increase in the model extraction status is shown as the number of colluding clients increases.





==> Model Extraction Paper/Introduction.tex <==
\section{Introduction}

Most cloud service providers (CSPs) now offer machine learning services that enable developers to train and host machine learning (ML) models on the cloud. 
Application developers or end users can access these models via prediction APIs on a pay-per-query basis. 
%
Recent work has showed that the hosted ML models are susceptible to model extraction attacks. 
Adversaries may abuse a model's query API and launch a series of intelligent queries spanning the input space to steal or replicate the hosted model, thus avoiding future query charges. Moreover, access to the model parameters can leak sensitive private information about the training data and facilitate evasion attacks especially if the model is utilized in security applications such as malware or spam classification~\cite{tramer,dwork2008differential,biggio2013evasion}.

Machine learning models generally encapsulate confidential information related to the problem domain. Additionally, the training data used to construct the model may be private and expensive to obtain. For instance, the business logic of an insurance firm is encoded in the model that predicts which customers are eligible for insurance.  Similarly, a significant number of expensive clinical trials and private health records may have been used to train a model that detects health issues in a patient. Therefore techniques to detect or prevent ongoing model extraction attacks are of significant importance to model owners and cloud service providers. Moreover, knowing the status of model extraction can help price queries as a function of extraction status and aid in making decisions regarding packaging models at an attractive price within a cloud subscription service. 
%regarding offering original models at an attractive price within a cloud subscription service. 

Prior work \cite{tramer} on model extraction showed that interpretable ML models such as linear and logistic regression can be replicated using a constant number of queries (of order of number of features) by solving a system of linear equations. For the non-interpretable machine learning models such as decision trees and neural networks, the number of queries needed to recover the model is variable and efficient attack strategies may be designed to successively steal the models over time. The focus of this work is to provide extraction status warnings for such machine learning models. In particular we focus on decision tree models used for classification although the proposed techniques are more broadly applicable to other machine learning models as well. We output warnings related to model extraction status for both single and multiple user query streams. In case of multiple users, our techniques can indicate the model extraction status in the presence of colluding adversaries. 
% Shed more light on the current methods - greedy, polynomial time, etc. 
%In order to detect In the presence of extraction attacks, we design a cloud-based \emph{extraction monitor} that provides status of the model extractions by observing the query and response streams from each user. 
%
\begin{figure}
    \centering
\includegraphics[width=\linewidth]{Images/sys_arc.jpg}
    \caption{System Architecture}
    \label{fig_architecture}
\end{figure}

Figure~\ref{fig_architecture} depicts the problem setting with different stakeholders. Model owners deploy their models on the cloud, which are accessed by end users via pay-per-query APIs. The CSP manages the query and response streams from each user to the deployed ML models. 
In order to detect extraction attacks from adversaries, we design a cloud-based \emph{extraction monitor} that continually informs model owners of the information recoverable by users based on the queries responded thus far. The extraction monitor has at least a partial visibility of the deployed model in order to provide such a status, with estimation quality improving with better visibility. We propose two different strategies that the monitor uses to infer the model learning rate of users. In the first strategy, the monitor computes the information gain of the users based on their queries received thus far. In order to do this, it uses a validation set supplied by the model owner that has a distribution similar to the training set. In the second strategy, the monitor maintains compact summaries of user queries and estimates their coverage of the input space relative to the partition induced by the source model. Both approaches can also provide joint extraction status corresponding to queries of user groups to understand the coverage of queries from colluding users. In particular the key contributions of this work are as follows: 
\begin{itemize}
\item{
We define a new metric to measure the information learnt by a decision tree with increasing amount of training data. The metric is based on entropy and measures the learning rate of an evolving decision tree with respect to a validation set provided by the model owner. It may be used to measure the information gained by adversaries with increasing number of API queries. We present a fast greedy algorithm that identifies the maximum information gained by any set of $k$ users among all users who have queried the model, which may be utilized in the presence of colluding adversaries.  
%the We define a new metric of information gain based on the entropy have said that we have ratio of information gain -- good metric for information gain 
%We have evaluated it with prior datasets (steak a good example). Attack strategy - path finding algorithm. Tramer's queries. Random queries. how its knowledge increases. 
}
\item{
We define an alternate metric that measures the information learnt by querying users by computing the coverage of the input space relative to the partitions induced by the source model owned by the owner. This approach maintains efficient summaries of user query streams and can identify the minimum number of users that have maximum information about the model in polynomial time.   
}
\item{We present experimental evaluation results for both approaches using open source datasets and decision trees deployed on BigML MLaaS platform. We present model extraction results for two attack strategies based on random queries and an intelligent path finding algorithm from prior work.}
%Our results show that (to do)}. 
\end{itemize} 


\subsubsection{Related Work. } Most of the existing work on model extraction focuses on different types of extraction or inversion attacks that divulge model parameters or sensitive private information about the training data to adversaries querying the model~\cite{dwork2008differential,ateniese2015hacking,tramer}. 
Also model extraction can facilitate evasion in applications such as spam filtering and anomaly or malware detection~\cite{huang2011adversarial,biggio2013evasion}. 
Although work has been done to analyze adversarial frameworks, we know of no prior work that estimates the extraction status of an adversary and provides warnings to model owners, which is the focus of our work. 
%our work is new in its kind, where we focus on quantifying extraction status of an adversary.


The balance of the paper is organized as follows. Section~\ref{sec:pf} presents the problem framework and section~\ref{sec:mew} presents two different approaches to compute model extraction status for both individual and colluding users. The experimental results with open source datasets are presented in section~\ref{sec:exp}. Lastly, conclusions and directions for future work are presented in section~\ref{sec:conclusions}.
%Related work is presented in section~\ref{sec:rw} before presenting conclusions and directions for future work in section~\ref{sec:conclusions}.





%Recently, several companies like Google, Amazon, BigML have started hosting machine learning models using their cloud platform. The models are typically owned by a service owner who uses the cloud owner's platform to serve its users. Users buy predictions from a deployed models to bypass the cost of infrastructure, training time, and expertise required to tune a model. Following are the role specifications:
%
%\begin{itemize}
%    \item {\textbf{Service Owner:}} Owns the model and training data, expects to sell the predictions of the model to users.
%    \item {\textbf{Cloud Owner:}} Owns the platform on which the model is deployed, manages the user interface.
%    \item {\textbf{User:}} Takes prediction outputs from the models and make payment for the service.
%\end{itemize}
%
%At times the service owner and cloud owner may be same entity or effectively considered the same when cloud owner get visibility of the training data and the model. But, for business reasons the cloud owner might not get full visibility of model deployed by the service owner, instead manages the interface for the model and hosts its users.
%
%A service owner usually chooses to keep model parameters hidden from the users, so that they query takes place in a black box manner with feature values as inputs to get predictions as outputs.  
%
%It has been established that input-output of a model can eventually reveal the model parameters to an adversarial user\cite{tramer2016stealing}. A user might build a model from the predictions outputs to avoid paying the charges for further queries or to extract the model with some malicious intent.  Since it is easy to track behaviour of individual user and identify the defaulters, a set of users might also come together and collude to get the model extracted. 
%
%In such a scenario, it could be helpful for a service owner to know the amount of information a user or a group of user is able to extract through the queries. Such information can help to decide the price of the queries in a variable manner for users, depending upon their extraction status.
%
%The proposed work enables a cloud owner having at least partial visibility of the deployed model, to estimate the extractions possible by individuals or group of users, based on their query history. The service owner gives visibility of the model to the cloud owner by the means of a validation set, which consists of query inputs and corresponding labels predicted by the hosted model. 
%
% The validation set can be negotiated between the cloud and service owner, given the fact that estimation quality would improve with better visibility. In case the cloud owner himself owns the service, the entire training set can be used as the validation set to get the best possible estimations of user extraction status.
%
%\begin{figure}
%    \centering
%\includegraphics[scale=0.36]{Images/sys_arc.jpg}
%    \caption{System Architecture}
%    \label{fig_architecture}
%\end{figure}
%
%Figure \ref{fig_architecture}, depicts the service architecture of the system. Where the cloud owner hosts the black box model of a service owner and its users. The user queries are sent to the hosted model and predictions are given back. But the cloud owner also maintains a summary $s_i$ for each user $i$, computed using the validation set provided by the service owner. The summaries are updated as the new query points comes from the users either one at a time or in a batch manner. 
%
%At any point of time the service owner might query the model extraction status of individual users or maximum extraction possible by $k$ colluding users. Or it might setup a warning to know when $90\%$ of the model is extracted by $k$ users. This work enables the cloud owner to efficiently able to answer such questions about the hosted model and its users.


==> Model Extraction Paper/Method.tex <==
\section{Method}

Given that the deployed model performing a classification task, in order to estimate the possible extraction by the users, the cloud owner who has complete visibility to the user inputs and labels predicted by the model, builds a decision tree for each user using their respective query history. The decision trees may be incrementally updated with each new query fired by the user or in a batch manner after certain interval of time. 

Decision trees are chosen to maintain user extraction status because they are easy to train, they can be build with few query points, they can be incrementally updated and combined. If the service owner chooses to deploy a classification model other than a decision tree, then a fair estimation about the knowledge of the users can obtained from the decision trees.  

The model extraction possible by the users are quantified using {\it information gain of a decision tree} which we define in the following way. 

 \subsection{Entropy of a validation set:}\cite{shannon2001mathematical} 
 Let $S$ be a set of training or validation elements, each element having an input $x$ with a class label $f(x)\in[k]$ assigned to it. Let $p_i$ denote the probability that a random element chosen from $S$ belongs to the class $i$. Then entropy of $S$ is defined by: 
  \begin{equation}
      Entropy(S)=-\sum\limits_{i=1}^{k}p_i \log{p_i}
  \end{equation}
  
  
  \subsection{Information gain ($IG$) of an attribute A:}\cite{quinlan1986induction} Let the set $S$ be partitioned using a categorical attribute $A$, then information gain of the attribute $A$ is defined as the reduction in entropy when we partition $S$ using values that attribute $A$ takes:
    	\begin{equation}
    	IG(S,A)=Entropy(S)-\sum\limits_{v\in val(A)}\frac{\abs{S_v}}{\abs{S}}Entropy(S_v)
    	\end{equation}
    	
We generalize this existing notion of information gain of an attribute to information gain of a decision tree, which enables us to measure the knowledge extraction by a user.

\subsection{Information gain of a decision tree:} Let a validation set $S$ be partitioned into disjoint sets $\{S_l\}$ by the leaf nodes of the decision tree $T$. The information gain of the tree is the reduction in entropy by partitioning $S$ using leaf nodes of $T$:
  \begin{equation}
      IG_{tree}(S,T)=Entropy(S)-\sum\limits_{l\in leaf(T)}\frac{\abs{S_l}}{\abs{S}}Entropy(S_l)
      \label{eq:info_gain}
  \end{equation}

Here, the entropy of a leaf node would computed with respect to the class labels given by the validation set. It should be observed that if a decision tree has rule sets close to the deployed decision tree, then each of the leaf node would segregate the validation data well and they would gather inputs mostly from single class of validation data, pushing the entropy of the leaf node close to zero. 

Similar behaviour from all the leaf nodes would result to a higher information gain for the tree. It can be observed that if we train a decision tree $T_S$ on the validation set $S$, without using constraint like maximum depth or minimum elements of split or use pruning, then all leave nodes will have elements from a single class, leading entropy of each of the leaf node $Entropy(S_l)$ to zero. So that information gain of the tree learned on $S$, would be equal to the entropy of $S$.
\begin{equation}
    IG_{tree}(S,T_S)=Entropy(S)       
\end{equation}

Using the above fact we prefer to represent model extraction by user $u$ as $IG_{tree}(S,T_u)/Entropy(S)$, often converted in a percentage form. Figure \ref{fig:acc_vs_info_gain} plots the accuracy of a decision a tree with respect to its information gain.

\begin{figure}
    \centering
\includegraphics[scale=0.19]{Images/acc_vs_info_gain.png}
    \caption{Accuracy vs Information Gain}
    \label{fig:acc_vs_info_gain}
\end{figure}

\begin{figure}
    \centering
\includegraphics[scale=0.3]{Images/tramer_vs_unif.png}
    \caption{Accuracy vs Information Gain}
    \label{fig:tramer_vs_unif}
\end{figure}

Given the metric, the service owner might be interested about the following queries:

\begin{enumerate}
    \item Information gain of each user
    
    \item Information gain of a given set of user

    \item Maximum information gain possible by any $k$ users

    \item Warning after the model extraction crosses a percentage $p$, by any $k$ possible users
\end{enumerate}

After building a decision tree on the query history of each user, the first query can directly answer using equation \ref{eq:info_gain}. One of the way to evaluate second query is take union of query points of the users and build a decision tree on it to get its information gain. The other way could be to combine the decision trees of each of the user in the set, and compute information gain of the combined decision tree. We have taken the first approach, for ease of implementation. Next we describe how to address the thrid query.

\subsection{Maximum information gain by any set of k users:} The service owner might like to know the maximum possible information that can be extracted by a set of $k$ colluding users. As there could be $n \choose k$ possible sets, the brute force method to measure the information gain of each set of users and to find the highest among them, as listed in algorithm \ref{alg:comb}, will have complexity exponential on $n$. 

To overcome this problem we take a greedy approach which at each step adds that decision tree that gives highest marginal gain over tree that has been built till now. Algorithm \ref{alg:greedy}, gives the pseudo-code for this greedy method. The algorithm needs a parameter $k$ and the query history of all $n$ users as input and gives a set of $k$ users and their information gain as the output. 
\begin{algorithm}
  	\caption{$combUserSelection$}
  	\label{alg:comb}
  	\begin{algorithmic}
  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
  		\REQUIRE validation set $S$, query hist. of $n$ users, parameter $k$
  		\ENSURE set of $k$ users, their information gain
  		\STATE $initial\_ent=Entropy(S)$
  		\STATE $pool=combinations(n,k)$
  		\FOR{$c \in pool$}
  		    \STATE $query\_points=[]$
  		    \FOR{$user \in c$}
  		        \STATE $query\_points=\{query\_points\cup query(user)\}$
  		    \ENDFOR
  		
  		\STATE $gain[c]=IG_{tree}(S,DecisionTree(query\_points))$
  		\ENDFOR
        \STATE $U=argmax(gain)$
        \STATE $max\_gain=\max(gain)$
        \RETURN $U, max\_gain/intial\_ent$
  	\end{algorithmic}
  \end{algorithm}
  
\begin{algorithm}
  	\caption{$greedyUserSelection$}
  	\label{alg:greedy}
  	\begin{algorithmic}
  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
  		\REQUIRE validation set $S$, query history Q, parameter $k$
  		\ENSURE set of $k$ users, its information gain
  		\STATE $initial\_ent=Entropy(S)$
  		\STATE $pool=[n], U=[\,]$
  		\FOR{$i\in [k]$}
  		    \STATE $x=-1, max\_gain=0$
  		    \FOR{$j \in pool$}
  		        \STATE $gain=IG_{tree}(S,DecisionTree(\{U \cup j\}))$
  		        \IF{$gain > max\_gain$}
  		        \STATE $x=j, max\_gain=gain$
  		        \ENDIF
  		    \ENDFOR
  		\IF{$x!=-1$}
  		    \STATE $U=\{U\cup x\}, pool=\{pool \setminus x\} $
  		\ENDIF
  		\ENDFOR
  		
        \RETURN $U, max\_gain/intial\_ent$
  	\end{algorithmic}
  \end{algorithm}

\subsection{Warning on model extraction:}
Given number of users on which we are looking for the extraction status, and a threshold algorithm \ref{alg:warn} generates the warning for the service owner. The interval after which the greedy algorithm is invoked might be decided upon the number of new queries that have arrived or it could be time interval.
\begin{algorithm}
  	\caption{$ExtractionWarning$}
  	\label{alg:warn}
  	\begin{algorithmic}
  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
  		\REQUIRE validation $S$, query historty $Q$, user $k$, threshold $p$
  		\WHILE{$gain<p$}
  		    \STATE $u, gain = greedyUserSelection(S,Q,k)$
  		    \STATE $wait()$
      	\ENDWHILE
      	\RETURN $warning\_message$

  	\end{algorithmic}
  \end{algorithm}
  
\subsection{Quality of the validation set:} The validation set is used to compute the information gain of the user decision trees. If the validation set contains less amount of information, for example, all the samples belonging to few specific classes, samples that are pocketed in the input space or  validation set consisting of less number of samples, then we could obtain incorrect estimations of information gain. In order to avoid that, the validation set may be assigned a information content score in the following way.

\begin{equation}
    Score(S)=IG_{tree}(Tr,DecisionTree(S))/Entropy(Tr)
\end{equation}

where $Tr$ is the training set confidential to service owner. The service owner scores the validation set using the above rule and hands the validation data over to the cloud owner. The score works as indicative of the confidence that should be rested upon the information gain estimates.


==> Model Extraction Paper/ModelExtAttack.tex <==
\section{Model Extraction Attack}
In MLaaS a Model Extraction Attack

==> Model Extraction Paper/ModelExtWarning.tex <==
\section{Model Extraction Warning}
\label{sec:mew}

%Our aim in this research is to genereate model extraction warning. 
Our goal is to design a cloud based monitor capable of providing model extraction status and warnings. 
Each query to a deployed ML model $f$ along with its response leaks a certain amount of information about the decision boundaries of the model to the user. 
After having made multiple queries, an adversarial user can train his own ML model $\hat{f}$ over the query-response set, which has a certain performance accuracy as compared to the source model $f$. 
%and construct a copy of the model $f$ 
%Our objective is to detect if any set of clients of size $k \ge 1$ jointly have the knowledge of the deployed ML model above a certain accuracy threshold. 
Our objective is to detect if any set of clients of size $k \ge 1$ can jointly reconstruct a model that yields an accuracy beyond a given threshold. 
The model owner may run the detection at fixed time intervals or after a certain number of queries have been answered by the deployed model.
In the subsequent sections, we focus on the decision tree models for classification and propose two strategies to detect model extraction by adversarial users. 
%In both the strategies we consider a separate module residing on the MLaaS cloud service provider monitoring the input queries of all the users. 

\subsection{Strategy 1: Model Extraction Warning using Information Gain. }
\label{subsec:s1}

\subsubsection{Initialization.~}
\label{subsubsec:s1init}
%In this strategy, we assume that the model owner has provided an extraction threshold $t$ and a validation set along with the ML model to the monitor. 
In this strategy, we assume that the model owner has provided an extraction threshold $t$ and a validation set to the monitor. The monitor observes the query response pairs of each user and incremently learns a local  decision tree based on these pairs. 
Let $S$ denote the validation set, with each element having an input $x$ and an associated class label $y\in[k]$. Let $p_i$ denote the probability that a random element chosen from $S$ belongs to the class $i$. 
Then the entropy of $S$ is defined by: 
\begin{equation}
      Entropy(S)=-\sum\limits_{i=1}^{k}p_i \log{p_i}
\end{equation}

\subsubsection{Information gain of a decision tree.~} 
\label{subsubsec:s1gain}
Recall that the information gain of an attribute is defined as the reduction in entropy of a training set when we partition it based on values that the attribute can take~\cite{quinlan1986induction}. 
%
%\subsection{Information gain ($IG$) of an attribute A:}\cite{quinlan1986induction} Let the set $S$ be partitioned using a categorical attribute $A$, then information gain of the attribute $A$ is defined as the reduction in entropy when we partition $S$ using values that attribute $A$ takes:
%    \begin{equation}
%    IG(S,A)=Entropy(S)-\sum\limits_{v\in val(A)}\frac{\abs{S_v}}{\abs{S}}Entropy(S_v)
%    \end{equation}
%   
%We generalize this existing notion of information gain of an attribute to information gain of a decision tree, which enables us to measure the knowledge extraction by a user.
%
%
We generalize this concept and define a metric called the \emph{information gain of a decision tree} $T$ with respect to a given validation set $S$. 
This metric is essentially computed by the monitor on its local decision tree to estimate the information gained by users based on their queries thus far. 
%This is an extension to the notion of information gain of an input attribute used to construct decision trees. 
By evaluating $S$ on $T$, let $S$ be partitioned into disjoint subsets $\{S_l\}$ by the leaf nodes of $T$. 
%The information gain of $T$ is defined as the reduction in entropy achieved by partitioning $S$ using leaf nodes of $T$:
The information gain of $T$ is defined as the reduction in entropy as follows: 
  \begin{equation}
      IG_{tree}(S,T)=Entropy(S)-\sum\limits_{l\in leaf(T)}\frac{\abs{S_l}}{\abs{S}}Entropy(S_l)
      \label{eq:info_gain}
  \end{equation}
%
%In Equation \ref{eq:info_gain}, the entropy of a leaf node ($Entropy(S_l)$) of the decision tree is computed using the original label of the validation elements.
where the entropy of a leaf node $l$ i.e. $Entropy(S_l)$ is computed using the original class labels of the validation elements.
Similarly, one can apply Eq.~\eqref{eq:info_gain} to compute the information gain of the model owners source decision tree $T_O$ as $IG_{tree}(S,  T_O)$. 
%\subsubsection{Information gain of the source ML model.~}
%\label{subsubsec:basegain}
%Similarly, we define the information gain of the model owners source decision tree $T_O$ ($IG_{tree}(S,T_O)$) using Equation \ref{eq:info_gain}.

\begin{figure}
    \centering
\includegraphics[scale=0.19]{Images/acc_vs_info_gain.png}
    \caption{Accuracy vs Information Gain}
    \label{fig:acc_vs_info_gain}
\end{figure}

Figure \ref{fig:acc_vs_info_gain} plots the accuracy of a user's decision a tree with respect to its information gain with increasing amount of training data. We observe that information gain accurately captures the learning rate of the user's model. 

%\begin{equation}
%    IG_{tree}(S,T_O)=Entropy(S)  
%    \label{eq:info_gain_source}
%\end{equation}
%
%Since the validation set provided by the model owner has a distribution similar to the training set, we expect the validation set to be classified accurately by $T_O$. Thus each leaf node would contain elements from a single class only and $Entropy(S_l) = 0~\forall l$ in eq.\eqref{eq:info_gain}, yielding eq.\eqref{eq:info_gain_source}. 

%The information gain of the model owner's ML model ($T_O$) is computed using the validation set. We assume that the validation set $S$ shared by Service Owner is part of the training set or it is classified accurately by $T_O$. 
%
%A decision tree which is trained using the validation set, without using constraints like maximum depth or minimum elements of split, will have leaf nodes containing elements from a single class only, leading to the entropy of each of the leaf node to zero ( i.e. $Entropy(S_l) = 0$) . So the maximum information gain of the tree learned on $S$, would be equal to the entropy of $S$. Hence the Information gain of the source model $T_O$ is given as, 
%
%\begin{equation}
%    IG_{tree}(S,T_O)=Entropy(S)  
%\end{equation}

\subsubsection{Model Extraction Status Per User.~}
\label{subsubsec:userstat} 
To compute the model extraction status for each user, the monitor trains a local decision tree $T_{u}$ based on all query-response pairs made by user $u$ to the source decision tree $T_O$. 
It uses the validation set $S$ to compute the information gain $IG_{tree}(S, T_{u})$ using eq.\eqref{eq:info_gain} and the extraction status as follows: 
%For each user we maintain all the queries and their responses that user had made to $T_O$ using the prediction api. Using these queries we train a decision tree for each user and compute their information gain ($IG_{tree}(S,T_{u_{i}}$) using the validation set as descibed above in Section \ref{subsubsec:s1gain}. 
\begin{equation}
    Extraction\_Status_{u} = \frac{IG_{tree}(S,T_{u})}{IG_{tree}(S,T_O)} * 100
\end{equation} 


For all the users whose $Extraction\_Status$ is more than the threshold $t$, a model extraction warning is generated and sent to the relevant model owners. 

\subsubsection{Model Extraction Status with Collusion.}
\label{subsubsec:usercoll}
%In a general scenario, the Service Owner would like to know if there is any set of $k$ colluding users which are trying to extract the deployed model. We can extend our existing approch to compute the model extraction warning in case of collusion.
In a general setting, a model owner would like to know if any $k$ of the $n$ users accessing the deployed model are colluding to extract it. We extend our existing approach to compute the model extraction warning in case of collusion as follows.

%In the brute force approach there will be $n \choose k$ possible combination of users. 
In a brute force approach, a monitor would need to compute the extraction status for all $n \choose k$ combinations of users. 
%Algorithm \ref{alg:comb} shows how we can find the set of users having maximum extraction of the deployed model using their combined query set. The complexity of this alogrithm is exponential in $n$.
Algorithm \ref{alg:comb} shows how the monitor can recover a set of $k$ users that have maximum knowledge of the deployed model using their combined query data. In this algorithm the function call $DecisionTree(query\_points)$ returns a decision tree trained over the provided $query\_points$.
\begin{algorithm}
  	\caption{$combUserSelection$}
  	\label{alg:comb}
  	\begin{algorithmic}
  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
  		\REQUIRE validation set $S$, query history $Q$, parameter $k$
  		\ENSURE set of $k$ users, their extraction status
  		\STATE $source\_gain = IG_{tree}(S,T_O)$
  		\STATE $pool=combinations(n,k)$
  		\FOR{$c \in pool$}
  		    \STATE $query\_points = \{\}$
  		    \FOR{$user \in c$}
  		        \STATE $query\_points=\{query\_points\cup Q[user]\}$
  		    \ENDFOR
  		
  		\STATE $gain[c]=IG_{tree}(S,DecisionTree(query\_points))$
  		\ENDFOR
        \STATE $U=argmax(gain)$
        \STATE $max\_gain=\max(gain)$
        \RETURN $U, (max\_gain/source\_gain)*100$
  	\end{algorithmic}
  \end{algorithm}
  
%To overcome the problem of exponential running time, we take a greedy approach, where at each step we select the user whose query set after comining with the queries of already selected users, gives the joint decision tree that has the highest information gain. Algorithm \ref{alg:greedy}, gives the pseudo-code for this greedy method. The algorithm needs a parameter $k$ and the query history of all $n$ users as input and gives a set of $k$ users and their extraction status as the output.  
The complexity of this algorithm is exponential in $n$.
To overcome the issue of exponential running time, we propose a greedy algorithm, where at each step the monitor selects that user whose query set in combination with the queries of selected users yields a decision tree that has the highest information gain. Algorithm \ref{alg:greedy} gives the pseudo-code for the greedy method. The algorithm needs a parameter $k$ and the query history of all $n$ users as input and returns a set of $k$ users that have the highest information along with their extraction status. 
%The model owner may run Algorithm \ref{alg:greedy} at fixed time intervals or after a certain number of queries have been answered by the deployed model.
\begin{algorithm}
  	\caption{$greedyUserSelection$}
  	\label{alg:greedy}
  	\begin{algorithmic}
  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
  		\REQUIRE validation set $S$, query history Q, parameter $k$
  		\ENSURE set of $k$ users, their extraction status
  		\STATE $source\_gain = IG_{tree}(S,T_O)$
  		\STATE $pool=[1, \cdots ,n], U=\{\}$
  		\FOR{$i = 1 to k$}
  		    \STATE $x=-1, max\_gain=0$
  		    \FOR{$j \in pool$}
  		        \STATE $gain = IG_{tree}(S,DecisionTree(Q[\{U \cup j\}]))$
  		        \IF{$gain > max\_gain$}
  		        \STATE $x=j, max\_gain=gain$
  		        \ENDIF
  		    \ENDFOR
  		\IF{$x!=-1$}
  		    \STATE $U=\{U\cup x\}, pool=\{pool \setminus x\} $
  		\ENDIF
  		\ENDFOR
  		
        \RETURN $U, (max\_gain/source\_gain) * 100$
  	\end{algorithmic}
  \end{algorithm}




\subsubsection{Quality of Model Extraction Warning. }
\label{subsubsec:s1quality}
%We have throughly experimented our approach to generate Model Extraction warning over a wide range of real datasets and presented our results in Section \ref{sec:exp}, 
%but nevertheless the quality of warning that is genereted will depened on how good the validation set fits the source ML model. In Section \ref{subsubsec:basegain} we assumed that the validiation set is classified accurately by $T_O$, but it is also possible that the validation set contains less amount of information in the sense that, all the samples in the validation set belong to a few classes. 
%In order to avoid that, the validation set may be assigned a information content score in the following way.
We present experimental results of model extraction warnings on real datasets in Section \ref{sec:exp}, which shed light on the accuracy of the extraction status. One of the factors that affects the quality of warning is the classification accuracy of the validation set. 
If the validation set is not accurately classified  by $T_O$ then, it may contains less information and all the samples in the validation set may belong to a few classes only. To avoid this, the validation set may be assigned an information content score as follows:
%
\begin{equation}
    Score(S)=IG_{tree}(Tr,DecisionTree(S))/Entropy(Tr)
\end{equation}
%
where $Tr$ is the training set confidential to the model owner. The model owner scores the validation set using the above rule before handing it to the monitor. The score can thus be used to assign a confidence value to the model extraction status estimates. 

%\begin{algorithm}
%  	\caption{$updateModelSummaries$}
%  	\label{alg:userSummary}
%  	\begin{algorithmic}
%  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
%  		\REQUIRE $UserID$, User query $q$
%  		\ENSURE create/update user summary
%  		\STATE $U\_Summary = getExistingSummaries()$
%  		\STATE $cID, leafID \leftarrow T_{S}.predict(q)$
%  		\STATE $S \leftarrow U\_Summary.Summary$
%  		\IF {$UserID \in U\_Summary.U$}
%  			\STATE $leaf\_info \leftarrow S[UserID].Leaf[leafID]$
%  			\FOR {$feature  in leaf\_info$}
%  				\STATE $feature[0] = min(q[feature],feature.min)$
%  				\STATE $feature[1] = max(q[feature],feature.max)$
%  			\ENDFOR	
%  		\ELSE
%  			\STATE $leaf\_info[f_t][2] \leftarrow newArray()$
%  			\FOR {$feature  in leaf\_info$}
%  				\STATE $feature[0] = q[feature]$
%  				\STATE $feature[1] = q[feature]$
%  			\ENDFOR
%  			\STATE $U\_Summary.add(UserID,leaf\_info)$
%		\ENDIF  		
%  	\end{algorithmic}
%  \end{algorithm}


\begin{algorithm}
  	\caption{$updateModelSummaries$}
  	\label{alg:userSummary}
  	\begin{algorithmic}
  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
  		\REQUIRE $UserID$, Query $q$
  		\ENSURE create/update user summary
  		\STATE $S = getExistingUserSummary(UserID)$
  		\STATE $classID, leafID \leftarrow T_{S}.predict(q)$
  		\IF {$S~ != Null $}
  			\STATE $leaf\_info \leftarrow S[leafID]$
  			\FOR {$feature  \in leaf\_info$}
  				\STATE $feature[0] = min(q[feature],feature.min)$
  				\STATE $feature[1] = max(q[feature],feature.max)$
  			\ENDFOR	
  		\ELSE
  			\STATE $leaf\_info[f_t][2] \leftarrow newArray()$
  			\FOR {$feature  \in leaf\_info$}
  				\STATE $feature[0] = q[feature]$
  				\STATE $feature[1] = q[feature]$
  			\ENDFOR
  		\ENDIF  		
  		\STATE $S[leafID] \leftarrow leaf\_info$
  	\end{algorithmic}
  \end{algorithm}
  
\subsection{Strategy 2: Model Extraction Warning using Compact User Summaries }
\label{subsec:s2}

%\begin{figure*}[ht!]
%            \includegraphics[width=.23\textwidth]{Images/Summary_1}\hfill
%            \includegraphics[width=.23\textwidth]{Images/Summary_2}\hfill
%            \includegraphics[width=.23\textwidth]{Images/Summary_3}\hfill
%            \includegraphics[width=.23\textwidth]{Images/Summary_4}\hfill            
%            \caption{Image B.}
% \end{figure*}


\begin{figure*}[!t]
  \centering
  \subcaptionbox{Class Boundaries of Source Model}[.23\linewidth][c]{%
    \includegraphics[width=.2\linewidth]{Images/Summary_1}}\quad
  \subcaptionbox{Summary of User A}[.23\linewidth][c]{%
    \includegraphics[width=.2\linewidth]{Images/Summary_2}}\quad
  \subcaptionbox{Summary of User B}[.23\linewidth][c]{%
    \includegraphics[width=.2\linewidth]{Images/Summary_3}}\quad
  \subcaptionbox{Combined Summary of User A and B}[.23\linewidth][c]{%
    \includegraphics[width=.2\linewidth]{Images/Summary_4}} 
  \caption{Model Summary Example}
  \label{fig:modelsummary}
\end{figure*}
\subsubsection{Initialization}
\label{subsubsec:s2}
%In this strategy we assume that the Service Owner outsources the ML model model along with the class probabilities $p_i, \forall i \in {y}$ and the hyper volume $vol_i, \forall i \in {y}$. If the source model is not a decision tree then Service Owner can train a decision tree along with the orignal model to compute hyper volume for each class. In Section \ref{sec:exp} we have shown, how this scheme works in the two cases i.e. whether the source model is a decision tree or not.
In the previous strategy, the monitor stores historical queries of all users accessing a model and maintains running decision trees on a combination of these queries. This can be computationally expensive if the number of users and queries are large. We now propose a novel approach wherein the monitor maintains and updates a compact model summary corresponding to each user with increasing number of queries. Each user's model summary effectively encompasses boundaries of regions within the feature space that the user may have learnt for each class. The monitor assess the coverage of summaries within their respective classes to compute the overall learning rate of a user. To assess the coverage accurately, the monitor uses the leaf id to which a query maps in the source decision tree in addition to the class label, which most decision tree APIs include in their response \footnote{This assumption is not new as authors in \cite{tramer} leverage it to mount model extraction attacks against decision trees.} (e.g. BigML). Additionally,  if there are $C$ classes, the monitor obtains the class probabilities from the model owner i.e. probability $p_i$ that an element from the training data belongs to class $C_{i}$ and the hyper volume of each class ($Class\_Vol_{i}$) (explained in the next subsections). 

%In this strategy we assume that the Service Owner outsources the ML model model along with the class probabilities $p_i, \forall i \in {y}$ and the hyper volume $vol_i, \forall i \in {y}$. If the source model is not a decision tree then Service Owner can train a decision tree along with the orignal model to compute hyper volume for each class. In Section \ref{sec:exp} we have shown, how this scheme works in the two cases i.e. whether the source model is a decision tree or not.

\subsubsection{Model Summary for each user. }
\label{subsubsec:s2extuser}
%For each user, we monitor all the queries and their responses that user had made to $T_O$. We assume that the query response also has the leaf id to which this query reaches in $T_O$ \footnote{This assumption is not new as the seminal work by authors in \cite{tramer}, have made same assumptions to mount a model extraction attack against Decision Trees.}.
%
%Suppose $t$ is the number of leaf nodes in $T_O$, $f_t$ is the number of features, then for each user we maintain the model summaries using a matrix of size $t \times f_t $.  Each entry in this matrix corresponds to the  constraint that the user has learned for a feature of a leaf node. 
For each user, the monitor observes all queries and their responses made to the deployed model $T_O$. The query response includes the class label and the leaf id to which a query maps in $T_O$. For a deployed decision tree model $T_O$ with $l_{t}$ leaf nodes and $f_t$ continuous input features\footnote{This strategy does not consider categorical features, since the notion of area or hyper-volume does not hold for such features}, each user's model summary is maintained as a matrix $M$ of size $l_t \times f_t $. The entry $M(i, j)$ corresponds to a linear constraint ($[min,max]$) on the feature $j$ that the user has learned for leaf node $i$. When a user issues a new query to $T_O$, its summary is updated using Algorithm \ref{alg:userSummary}. 

For ease of exposition, we present a simple example. Consider a deployed decision tree model with $f_t=2$ training features, $t=7$ leaf nodes, and $5$ classes. Let the class labels and decision boundaries created by the leaf nodes be as shown in Figure~\ref{fig:modelsummary}(a). Let two users $A$ and $B$ query this deployed model. Then, Figure \ref{fig:modelsummary}(b) and \ref{fig:modelsummary}(c) show the user queries as points in the feature space along with the rectangular summaries stored by the monitor for each leaf node. 

%\begin{algorithm}
%  	\caption{$extractionStatusPerUser$}
%  	\label{alg:userExtStat}
%  	\begin{algorithmic}
%  		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%  		\renewcommand{\algorithmicensure}{\textbf{Output:}}
%  		\REQUIRE Class probabilities $p_i$, source model hyper-volume $vol_i$, leaf ID and class mapping $M$, Classes $C$
%  		\ENSURE User Extraction Status Percentage
%  		\STATE $U\_Summary = getExistingSummaries()$
%		\STATE $S \leftarrow U\_Summary.Summary$
%		\STATE $ExtPer = []$
%		\FOR {$UserID \in U\_Summary.U$}
%			\STATE $LeafArea = []$
%			\FOR {$leaf\_info \in S[UserID].Leaf$}
%				\STATE $area = 1$	
%				\FOR {$feature  in leaf\_info$}
%					\IF {$feature[0] != feature[1]$}
%						\STATE $area = area * abs(feature[1] - feature[0])$
%					\ENDIF
%				\ENDFOR
%				\IF {$area != 1$}
%					\STATE $LeafArea.append(leaf.LeafID,area)$
%				\ENDIF
%			\ENDFOR
%			\STATE $ClassArea = []$
%			\FOR {$classID \in C$}
%				\STATE $classArea = 0$
%				\FOR {$leaf \in LeafArea$}
%					\IF {$M(leaf.LeafID) == classID$}
%						\STATE $classArea += leaf.area$
%					\ENDIF
%				\ENDFOR
%				\STATE $ClassArea.append(classID,classArea)$
%			\ENDFOR
%			\STATE $userExtPer = 0$
%			\FOR {$cInfo \in ClassArea$}
%				\STATE $c \leftarrow cInfo.classID$
%				\STATE $a \leftarrow cInfo.classArea$
%				\STATE $userExtPer += ((a / vol_{c}) * 100)$
%			\ENDFOR
%			\STATE $ExtPer.append(UserID,userExtPer)$
%		\ENDFOR			
%  	\end{algorithmic}
%  \end{algorithm}
  
 \subsubsection{Model Extraction Status Per User. }
\label{subsubsec:s2extstat}
%Let us assume that the source model is a decision tree and there are only two features on which the source model is trained (we will remove these assumptions later in this section and provide a general stategy). 
%
%Figure \ref{fig:modelsummary}(a) shows the class labels on the decision boundary of the source model created by the leaf nodes. 
%Lets say there are two users $A$ and $B$ quering this deployed model. As shown in Figure \ref{fig:modelsummary}(b) and \ref{fig:modelsummary}(c), we only store the end-points of the constraints for each of the leaf nodes for all the users. When a user issues a new query to the deployed model $T_O$, its summary is updated as using Algorithm \ref{alg:userSummary}.
 
%To compute model extraction status we use the model summary of that user. From the summary each leaf is identified one by one and the constraints over the features of that leaf are used to compute the area for that leaf \footnote{In case of $f_t > 3$ hypervolume is computed.}. Then we add the area corresponding to the leaf that belong to same class, and then the extraction per class is computed using the area per class of the source model ($vol_i$), finally the model extraction for the user is given by combining the per class extraction percentage using the class probabilities $p_i$. Algorithm \ref{alg:userExtStat} shows the steps for computing model extraction status per user.

To compute model extraction status for a user, the monitor computes the area (equivalently hypervolume when $f_t >= 3$) corresponding to each leaf $i$ using entries $M(i, j)~\forall j$ in the model summary matrix as follows,

\begin{equation}
Leaf\_Vol_{i} = \prod_{j \in f_t } abs(M(i,j).max - M(i,j).min) ~~\forall i \in l_t
\end{equation}

Then the area of each class is computed by aggregating leaves of the same class and the extraction percentage per class is computed using the ratio of the area in the model summary to the area per class of the source model (Note that the monitor has access to the hypervolume of each class in the source model) as shown in Equation \ref{eq:s2ExtPerClass}.

\begin{equation}
\label{eq:s2ExtPerClass}
Ext\_Per\_Class_i = \frac{\sum_{l \in C_i}(Leaf\_Vol_{i})}{Class\_Vol_i} ~~ \forall i \in C
\end{equation}

Finally, the extraction status of a user is computed as a weighted sum of per-class extraction percentages by weighing each term with the class probability $p_i$. 

\begin{equation}
\label{eq:s2extstatus}
Extraction\_Status = \sum_{i \in C}(p_i * Ext\_Per\_Class_i)
\end{equation}

%All the users whose extraction status is more than the extraction theshold are flagged as the potential adversaries of the system and the service owner is informed with their model extraction status.
For all the users whose extraction status is above the threshold $t$, a model extraction warning is generated and sent to the relevant model owners. 


  
\subsubsection{Model Extraction Status with Collusion. }
\label{subsubsec:s2coll}
%As discussed for Strategy 1 in Section \ref{subsubsec:usercoll}, model owner might be interested to know if any specific set of $k$ users are colluding for model extraction. Here again we can use the greedy strategy to select the best set of $k$ users with maximum knowledge of the model in polynomial time. The only difference in the algorithm here will ocuur in the user selection step, here the user whose addition gives the maximum hyper-vol for the collusion is selected instead of using the Information Gain metric. In Section \ref{sec:exp} we have provided results for the single user and collusion cases.
As discussed for Strategy 1 in Section \ref{subsubsec:usercoll}, a model owner may be interested to know the joint extraction of a set of $k$ users who may be colluding. Here again we use a greedy approach to compute the set of $k$ users with maximum knowledge of the model in polynomial time. The only difference in the algorithm is that during the the user selection step, the monitor chooses a user such that the combined model summary has the maximum hypervolume instead of maximum Information Gain. Fig.~\ref{fig:modelsummary}(d) illustrates an example of combining the model summaries of two users. The next section presents experimental results of extraction status for both single and collusion of adversarial users. 











==> Model Extraction Paper/Prelim.tex <==
\section{Preliminaries}

==> Model Extraction Paper/ProblemFW.tex <==
\section{Problem Framework}
\label{sec:pf}
%supervised learning 
%Only Classification Alogorithms
% Black Box models


%The MLaaS paradigm allows Data Owners to train a ML model over their training set and outsource the learned model to cloud service providers. 
The MLaaS paradigm allows ML developers to train a model based on their data and deploy it on the cloud. The end users query the model using its prediction APIs. We regard an ML model as a function $f : X \rightarrow y$ that maps a d-dimensional input feature vector $x_i \in X$ to a prediction $y_i \in y$, which is a categorical variable. 
%which may be categorical or a continuous variable. 
%\subsection{Model Extration Attack}
%\label{subsec:mea}

\vspace{1mm}\noindent{\bf Model Extration Attack.~} In the case of a model extraction attack, an adversary abuses the prediction API of a model $f$ and attempts to learn a model $\hat{f}$ that achieves similar performance as $f$. 

%\subsection{Adversary Model}
%\label{subsec:AdvModel}
\vspace{1mm}\noindent{\bf Adversary Model.~}
%In our work, the adversary can be a single client or a group of colluding clients, having access to the blackbox ML model prediction api. 
In our work, the adversary can be a single user or a group of colluding users that have access to the ML model's prediction API. Furthermore adversaries may have knowledge of the model type (e.g. Decision Tree or Logistic Regression), or the kind of data it is trained upon with the objective of learning the ML model's parameters via a sequence of intelligent queries. 
%or the kind of data it is trained upon, with the objective of learning the ML model's parameters. 
% TODO: define the above more clearly

%\subsection{Performance Metrics}
\vspace{1mm}\noindent{\bf Performance Metrics.~}
%We use the following metric to show the closeness of the models learned by the users with respect to the deployed model.
In order to compare the performance of a model $\hat{f}$ learnt by an adversary with respect to the deployed source model $f$, we compute the following metrics \cite{tramer}. Note that the monitor does not have access to any models learnt by the adversaries, but simply their queries. 
\subsubsection{$1-R_{test}:$}
While building the source model $f$, the model owner generally splits the dataset into train and test sets. We use this test data set $T$ to compare the performance of the source and learnt models. 
%On each run of the simulation $20\%$ of instances of the dataset are selected randomly and kept aside. Input part these instances feed to deployed model to get label predictions. Original labels that came with dataset are discarded. This constructs the test data $T$ for $R_{test}$, which measures the fraction of instances where the user model $\hat{f}$ predictions are different from the prediction of the deployed model $f$. That is,
\begin{equation}
    R_{test} =\dfrac{1}{\abs{T}} \sum_{t\in T} I(\hat{f}(x^{(t)})\neq f(x^{(t)}))
\end{equation}
where $I$ denotes the indicator function. Thus $1-R_{test}$ represents the accuracy of an adversary's model with respect to the deployed model.

\subsubsection{$1-R_{unif}:$}
In addition to testing the adversary's model on the test data set that follows a specific distribution, we also test the learnt model against a data set $U$ that is generated uniformly from the input feature space. 
\begin{equation}
    R_{unif} =\dfrac{1}{\abs{U}} \sum_{t\in U} I(\hat{f}(x^{(t)})\neq f(x^{(t)}))
\end{equation}
Thus $1-R_{unif}$ represents another metric to evaluate the performance an adversary's model as compared to a deployed model. 

%\subsection{Preliminaries}
%\label{subsec:prelim}
%
%Define Entropy and Information Gain here \\
%Define $1-R_{test}$ and $1-R_{unif}$ \\
%Hyper volume \\


==> Model Extraction Paper/RelWork.tex <==
\section{Related Work}
\label{sec:rw}

Most of the existing work on model extraction focuses on different types of extraction or inversion attacks that divulge model parameters or sensitive private information about the training data to adversaries querying the model~\cite{dwork2008differential,ateniese2015hacking,tramer}. 
Also model extraction can facilitate evasion in applications such as spam filtering and anomaly or malware detection~\cite{huang2011adversarial,biggio2013evasion}. 
Although work has been done to analyze adversarial frameworks, we know of no prior work that estimates the extraction status of an adversary and provides warnings to model owners, which is the focus of our work. 
%our work is new in its kind, where we focus on quantifying extraction status of an adversary.



==> ModelExtAttack.tex <==
\section{Model Extraction Attack}
In MLaaS a Model Extraction Attack

==> Prelim.tex <==
\section{Preliminaries}

==> RelWork.tex <==
\section{Related Work}
\label{sec:rw}

Most of the existing work on model extraction focuses on different types of extraction or inversion attacks that divulge model parameters or sensitive private information about the training data to adversaries querying the model~\cite{dwork2008differential,ateniese2015hacking,tramer}. 
Also model extraction can facilitate evasion in applications such as spam filtering and anomaly or malware detection~\cite{huang2011adversarial,biggio2013evasion}. 
Although work has been done to analyze adversarial frameworks, we know of no prior work that estimates the extraction status of an adversary and provides warnings to model owners, which is the focus of our work. 
%our work is new in its kind, where we focus on quantifying extraction status of an adversary.


